The Overthinker's DIET: Cutting Token Calories with DIfficulty-AwarE Training

Recent large language models (LLMs) exhibit impressive reasoning but often over-think, generating excessively long responses that hinder efficiency. We introduce DIET ( DIfficulty-AwarE Training), a framework that systematically cuts these "token calories" by integrating on-the-fly problem difficulty into the reinforcement learning (RL) process. DIET dynamically adapts token compression strategies by modulating token penalty strength and conditioning target lengths on estimated task difficulty, to optimize the performance-efficiency trade-off. We also theoretically analyze the pitfalls of naive reward weighting in group-normalized RL algorithms like GRPO, and propose Advantage Weighting technique, which enables stable and effective implementation of these difficulty-aware objectives. Experimental results demonstrate that DIET significantly reduces token counts while simultaneously improving reasoning performance. Beyond raw token reduction, we show two crucial benefits largely overlooked by prior work: (1) DIET leads to superior inference scaling. By maintaining high per-sample quality with fewer tokens, it enables better scaling performance via majority voting with more samples under fixed computational budgets, an area where other methods falter. (2) DIET enhances the natural positive correlation between response length and problem difficulty, ensuring verbosity is appropriately allocated, unlike many existing compression methods that disrupt this relationship. Our analyses provide a principled and effective framework for developing more efficient, practical, and high-performing LLMs.

==> sections/data_perspective.tex <==
\section{Data Perspective: Selecting the Right Ingredients}
\label{sec:data-perspective}

In this section, we investigate how the difficulty distribution of training data influences token compression effectiveness. While prior studies have demonstrated that curating training data based on difficulty significantly impacts overall RL performance \citep{skywork-or1-2025, DBLP:journals/corr/abs-2503-14476, wang2025dump}, its influence on token compression effectiveness remains largely underexplored. We demonstrate that the difficulty profile of the training data not only influences final performance but also critically dictates how effectively token compression can be achieved. While token compression techniques are often applied uniformly across tasks, we hypothesize that the inherent complexity of different reasoning problems fundamentally alters how models respond to token reduction incentives. Our analysis seeks to answer: \textit{Does applying the same compression technique to data subsets of varying difficulty levels lead to different performance-efficiency outcomes?} Understanding this relationship is crucial, as it could suggest that carefully selecting the "ingredients", i.e., the training examples based on their difficulty, is a key first step in an effective compression recipe.

\subsection{Experimental Setup}
\label{sec:data-perspective-setup}

To isolate the effect of data difficulty, we conduct controlled experiments where the compression method remains constant while the difficulty profile of the training data varies. We utilize the training dataset from DeepScaleR~\citep{deepscaler2025}, featuring problems of high quality and diverse complexity.

\textbf{Difficulty-Based Dataset Partitioning.}
We first quantify problem difficulty using the framework from \cref{sec:preliminary-difficulty}. Specifically, we employ the R1-distilled Qwen 1.5B model~\citep{DBLP:journals/corr/abs-2501-12948} to generate $N=8$ responses for each training question. We calculate the estimated correctness $\hat{C}(x, \pi_{1.5B})$ for each question $x$ and partition the training dataset into three equally sized strata of 9k questions based on this initial assessment: \textit{Easy} ($\hat{C}(x) \in [0.75, 1.0]$), \textit{Medium} ($\hat{C}(x) \in [0.25, 0.75)$), and \textit{Hard} ($\hat{C}(x) \in [0, 0.25)$). Additionally, we create a \textit{Random} split by randomly sampling an equal-sized subset from the full dataset, representing training on a typical mixed-difficulty distribution without specific selection.

\textbf{Fixed Token Compression Baseline.}
We apply a basic token compression method across all training runs on these data subsets. We adopt the token penalty introduced in Kimi 1.5~\citep{team2025kimi}, designed to reward conciseness for correct answers relative to other samples for the same prompt. For each prompt $x$ during training, we sample $N=8$ responses $\{y_i\}_{i=1}^N$. The token-related reward component for response $y_i$ is given by:
\begin{equation}
r_{\text{token}}(y_i, \{y_j\}_{j=1}^N) =
\begin{cases}
    \gamma_i, & \text{if } \mathbb{I}(y_i\text{ is correct}) = 1 \\
    \min(0, \gamma_i), & \text{if } \mathbb{I}(y_i\text{ is correct}) = 0
\end{cases}
\label{eq:kimi_penalty}
\end{equation}
where $\gamma_i = 0.5 - \frac{L(y_i) - \min_{j} L(y_j)}{\max_{j} L(y_j) - \min_{j} L(y_j) + \epsilon}$. Here, $L(y_i)$ is the length of response $y_i$, and the denominator normalizes the length relative to the minimum and maximum lengths among the $N=8$ responses sampled for prompt $x$ in the current batch ($\epsilon$ prevents division by zero). This reward encourages correct responses to be closer to the minimum length observed for that prompt. The overall reward is $r(x, y_i) = r_{\text{outcome}}(y_i) + \lambda \cdot r_{\text{token}}(y_i, \{y_j\}_{j=1}^N)$, where $r_{\text{outcome}}(y_i)$ is the binary correctness and $\lambda$ is a fixed hyperparameter controlling the penalty strength, kept identical across all runs.

\textbf{Training and Evaluation.} We train the R1-Distilled Qwen 1.5B and 7B models separately on each of the four data splits (Easy, Medium, Hard, Random) using the GRPO algorithm with the reward function defined above and consistent hyperparameters. For evaluation, we follow~\citet{DBLP:journals/corr/abs-2501-12948} and sample 64 times to estimate Pass@1 for AIME 2024, and sample 20 times for other benchmarks. More details for training and evaluation can be found in \cref{?}.

\subsection{Results: Medium Difficulty Yields the Best Trade-off}
\label{sec:data-perspective-results}

Table \ref{tab:difficulty-split-results-1.5b} presents the performance (Pass@1) and average response length on various math reasoning benchmarks for the Qwen 1.5B model trained on different difficulty splits.

\begin{table}[t]
\centering
\caption{Performance (Pass@1, \%) and average token length of R1-Distilled Qwen 1.5B trained on different difficulty splits using a fixed token compression method. Results show that training on the Medium difficulty split yields the best performance-efficiency trade-off. Best performance per metric is bolded, second best is underlined.}
\label{tab:difficulty-split-results-1.5b}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{l cc cc cc cc cc cc}
\toprule
\multirow{2}{*}{\raisebox{-0.6\height}{\makecell[l]{\textbf{Training Split}\\(\textit{Difficulty})}}} & \multicolumn{2}{c}{\textbf{MATH 500}} & \multicolumn{2}{c}{\textbf{AIME 2024}} & \multicolumn{2}{c}{\textbf{AMC 2023}} & \multicolumn{2}{c}{\textbf{Olympiad.}} & \multicolumn{2}{c}{\textbf{Minerva}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
 & P@1 & Tok & P@1 & Tok & P@1 & Tok & P@1 & Tok & P@1 & Tok & P@1 & Tok \\ \midrule
Original Model & 82.1 & 5534 & 28.5 & 16590 & 62.7 & 10615 & 43.5 & 11587 & 26.0 & 7076 & 48.6 & 10280 \\
\midrule
Easy   & \underline{79.3} & 1726 & \underline{27.1} & 8491 & \underline{63.6} & 4153 & \textbf{42.5} & 4730 & 25.0 & 1385 & 47.5 & 4097 \\
Medium & \textbf{80.6} & \underline{1776} & \textbf{27.2} & \underline{7280} & \textbf{63.9} & \underline{3895} & \underline{41.8} & \underline{4168} & \textbf{25.6} & \underline{1455} & \textbf{47.8} & \underline{3715} \\
Hard   & 63.5 & \textbf{750} & 6.8 & \textbf{2254} & 36.2 & \textbf{1156} & 26.0 & \textbf{1216} & 17.6 & \textbf{709} & 30.0 & \textbf{1217} \\
Random & 74.7 & 1429 & 21.7 & 7517 & 60.3 & 3808 & 38.9 & 3823 & 23.0 & 1124 & \underline{43.7} & 3540 \\ \bottomrule
\end{tabular}
}
\end{table}

The results clearly demonstrate that the difficulty profile of the training data significantly impacts the outcome of token compression. Training solely on \textit{Easy} problems leads to relatively high performance on some benchmarks but results in the longest average response lengths, indicating the model doesn't learn strong conciseness habits when problems are simple. Conversely, training on \textit{Hard} problems drastically reduces token counts (average 1217 tokens) but severely degrades performance across all benchmarks. This suggests that applying length penalties is detrimental when the model struggles with the core task, the model turns to minimize the token penalty instead of improving task performance. Notably, training on the \textit{Medium} difficulty split achieves the best overall average performance while maintaining a considerably reduced average token length compared to the Easy split. It strikes the most effective balance between maintaining reasoning capability and reducing verbosity. The \textit{Random} split performs reasonably but is generally surpassed by the Medium split in achieving the best trade-off, highlighting the benefit of curated difficulty selection over simple random sampling. Results for R1-distilled Qwen 2.5 7B models are presented in \cref{?}, where a similar conclusion can be drawn.

\subsection{Generalization of Difficulty Categorization Across Model Sizes}
\label{sec:data-perspective-generalization}

A crucial question is whether difficulty levels identified by a smaller model (1.5B) remain relevant when training a larger model. To test this, we trained the larger R1-Distilled Qwen 7B model using the exact same data splits derived from the 1.5B model's initial assessment.

Table \ref{tab:difficulty-split-results-7b} shows the results. We observe a similar pattern: the 7B model trained on the \textbf{Medium} difficulty split (as defined by the 1.5B model) again achieves the most favorable balance, yielding the highest average Pass@1 performance while keeping token lengths significantly lower than training on the Easy split. This demonstrates that difficulty categorization derived from a smaller, more efficient model can effectively guide data selection for training larger, more capable models, making this "ingredient selection" process practical.

{\color{red} table}
\begin{AIbox}{Takeaways for Data Perspective}
In token compression training, curating training data for medium difficulty yields the best performance-token trade-offs. And this difficulty assessment generalizes across model scales: difficulty estimated by a smaller model can effectively guide data selection for training larger models.
\end{AIbox}


==> sections/dynamic_perspective.tex <==
% \section{Training Dynamics Perspective: Cyclical Compression and Relaxation}
% \label{sec:training-dynamics}
% The previous sections focused on defining effective, difficulty-aware token penalties applied consistently at each training step. However, maintaining a constant, strong compression pressure throughout training might not be optimal. It could potentially trap the model in suboptimal solutions where reasoning quality is sacrificed for brevity, or hinder the model's ability to consolidate learning after aggressive length reduction phases. We hypothesize that varying the intensity of the compression incentive over time, implementing cycles of stronger compression followed by periods of relaxation, might foster more robust learning and lead to better final performance-efficiency trade-offs. This approach mirrors metabolic cycles – alternating phases of \textit{dieting} (strong compression) with phases of \textit{refueling} (relaxed compression) to allow for adaptation and recovery.

% \subsection{Cosine Modulation for Penalty Strength}
% \label{sec:dynamics-method}

% To implement these cycles, we introduce a time-varying modulation factor, $c(t)$, based on a cosine function. At training step $t$, this factor is:
% \begin{equation}
%  c(t) = 0.5 \left(1 + \cos\left(\frac{2\pi t}{T}\right)\right).
%  \label{eq:cosine_modulation_factor}
% \end{equation}
% Here, $T$ is the period of one cycle in training steps. This factor $c(t)$ smoothly oscillates between 1 (at $t=0, T, 2T, \dots$, representing peak compression) and 0 (at $t=T/2, 3T/2, \dots$, representing maximum relaxation). This factor $c(t)$ then directly multiplies the penalty coefficient determined by the chosen adaptive method: (1) For Adaptive Weighting (\cref{sec:reward-shaping-adaptive-weighting}), the overall coefficient becomes $c(t) \cdot \lambda_{\text{eff}}(x, \pi_\theta)$, using $\lambda_{\text{eff}}$ from \cref{eq:effective_lambda}. (2) For Dynamic Target (\cref{sec:reward-shaping-dynamic-target}), the overall coefficient becomes $c(t) \cdot \lambda_{\text{base}}$, using $\lambda_{\text{base}}$ from \cref{eq:reward_dynamic_target}.
% This cyclically scales the penalty strength, implementing the desired compress-relax dynamic.


% \subsection{Experimental Evaluation}
% \label{sec:dynamics-experiments}

% \begin{table}[ht]
% \centering
% \caption{Comparing Cyclical Penalty Strength (Cosine Modulation) with Constant Penalty Strength Adaptive Methods on R1-Distilled Qwen 1.5B.}
% \label{tab:dynamics-results-1.5b}
% \resizebox{1.0\textwidth}{!}{%
% \begin{tabular}{l c c c c c c c c c c | c c}
% \toprule
% \multirow{2}{*}{\raisebox{-0.6\height}{\textbf{Method}}} & \multicolumn{2}{c}{\textbf{MATH 500}} & \multicolumn{2}{c}{\textbf{AIME 2024}} & \multicolumn{2}{c}{\textbf{AMC 2023}} & \multicolumn{2}{c}{\textbf{Olympiad.}} & \multicolumn{2}{c|}{\textbf{Minerva}} & \multicolumn{2}{c}{\textbf{Average}} \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
%  & P@1 & Tok & P@1 & Tok & P@1 & Tok & P@1 & Tok & P@1 & Tok & P@1 & Tok \\ \midrule
% Base Model                  & 0.821          & 5534   & 0.285          & 16590 & 0.627          & 10615 & 0.435          & 11587 & 0.260          & 7076  & 0.486          & 10280 \\ \midrule
% Adaptive Weighting (\textit{Constant $\lambda$}) & 0.781 & 1835   & 0.270          & 8166  & 0.639          & 4335  & \textbf{0.419} & 4806  & 0.256          & 1570  & 0.473          & 4142 \\
% Adaptive Weighting (\textit{Cosine Mod.})  & \textbf{0.827} & 2877   & \textbf{0.322} & 10255 & \textbf{0.644} & 5819  & \textbf{0.437} & 6494  & \textbf{0.266} & 3171  & \textbf{0.499} & 5723 \\
% \midrule
% Dynamic Target (\textit{Constant $\lambda$})   & 0.801          & 1546   & 0.270          & 6795  & 0.636          & 3467  & 0.417          & 3815  & 0.249          & 1126  & 0.475          & 3350 \\
% Dynamic Target (\textit{Cosine Mod.})\\
% \bottomrule
% \end{tabular}%
% }
% \end{table}


% Table \ref{tab:dynamics-results-1.5b} presents the results. 

% {\color{red}...}

% \begin{AIbox}{Takeaways for Training Dynamics Perspective}
% Modulating the overall token penalty strength cyclically (e.g., via \textbf{cosine modulation}) influences the performance-efficiency trade-off. Preliminary results suggest cyclical schedules can help recover reasoning performance lost during compression, potentially reaching near-base model accuracy, but at the cost of higher average token counts compared to constant adaptive penalties. This offers another tuning dimension for balancing performance and efficiency.
% \end{AIbox}

